How to synchronize Digital Twins? A Communication Performance Analysis

Synchronization is fundamental for mirroring real-world entities in real-time and supporting effective operations of Digital Twins (DTs). Such synchronization is enabled by the communication between the physical and virtual realms, and it is mostly assumed to occur in real-time. However, this is not the case, as real-life scenarios witness performance degradation that may lead to synchronization problems. Hence, as such a problem has yet to be thoroughly analyzed in the literature, this work attempts to uncover potential challenges by emulating and analyzing the DT traffic flows in networks of different scales, for different communication protocols, and with various flow configurations. We propose a Twin Alignment Ratio metric to evaluate the synchronization performance to achieve this goal. Consequently, the findings reveal the interplay of network infrastructure, protocol selection, and twinning rate on synchronization and performance.

==> deleted.tex <==
\subsection{Digital Twin}
Digital Twins (DTs) are defined as real-time replicas of physical devices which contain real-time two-way communication. DTs enable real-time monitoring,  analysis, online what-if analysis, and data-driven decision-making. Moreover, DTs can be categorized under Edge Digital Twin and Cloud Digital Twin based on the deployment conditions. 

An Edge DT is a decentralized approach in which the DT resides in spatially close proximity to the physical devices that are being twinned. This enables low-latency communication and can guarantee prompt decision-making. Therefore, they are suited for autonomous control mechanisms which do not require extensive processing. 

On the other hand, Cloud DT is a centralized model which benefits from the scalability and resources of the cloud environment. These DTs can be utilized for complex, comprehensive analysis of current and historical data. Consequently, Cloud DTs are especially suited for non-time-critical applications that prioritize advanced data processing and long-term insights.

